Numerical simulations with a first order BSSN formulation of Einstein's field equations

We present a new fully first order strongly hyperbolic representation of the BSSN formulation of Einstein's equations with optional constraint damping terms. We describe the characteristic fields of the system, discuss its hyperbolicity properties, and present two numerical implementations and simulations: one using finite differences, adaptive mesh refinement and in particular binary black holes, and another one using the discontinuous Galerkin method in spherical symmetry. The results of this paper constitute a first step in an effort to combine the robustness of BSSN evolutions with very high accuracy numerical techniques, such as spectral collocation multi-domain or discontinuous Galerkin methods.

==> Preamble.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This is all for the hyperref package, and nice colors
\RequirePackage{ifpdf}
\ifpdf
%\usepackage{pdfsync}
\usepackage[backref=page, colorlinks, hyperindex, plainpages=false, %
bookmarksnumbered, pdfpagemode=UseNone, hyperfigures=true]{hyperref}
\usepackage{thumbpdf}
\renewcommand*{\backref}[1]{}
\renewcommand*{\backrefalt}[4]{% 
  \ifcase #1 { } \or (Cited on page~#2.) \else %
  (Cited on pages~#2.) \fi %
}
\else
\usepackage[colorlinks, pdfborder={0 0 0}, hyperindex,%
plainpages=false]{hyperref}
\fi
\definecolor{ChapterColor}{rgb}{0.510, 0.118, 0.000}
\definecolor{LinkColor}   {rgb}{0.741, 0.173, 0.000}
\definecolor{CiteColor}   {rgb}{0.000, 0.502, 0.118}
\definecolor{UrlColor}    {rgb}{0.000, 0.212, 0.800}
\hypersetup{linkcolor=LinkColor}
\hypersetup{citecolor=CiteColor}
\hypersetup{urlcolor=UrlColor}
%\hypersetup{pdflang={English}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

